ClustML: A Measure of Cluster Pattern Complexity in Scatterplots Learnt from Human-labeled Groupings

Visual quality measures (VQMs) are designed to support analysts by automatically detecting and quantifying patterns in visualizations. We propose a new VQM for visual grouping patterns in scatterplots, called ClustML, which is trained on previously collected human subject judgments. Our model encodes scatterplots in the parametric space of a Gaussian Mixture Model and uses a classifier trained on human judgment data to estimate the perceptual complexity of grouping patterns. The numbers of initial mixture components and final combined groups. It improves on existing VQMs, first, by better estimating human judgments on two-Gaussian cluster patterns and, second, by giving higher accuracy when ranking general cluster patterns in scatterplots. We use it to analyze kinship data for genome-wide association studies, in which experts rely on the visual analysis of large sets of scatterplots. We make the benchmark datasets and the new VQM available for practical use and further improvements.

==> biblio_bib <==
@STRING{AVI = {Proc. Int. Conf. on Advanced Visual Interfaces (AVI)}}
@STRING{BELIV = {Proc. Workshop on Beyond Time and Errors on Novel Evaluation Methods for Visualization (BELIV)}}
@STRING{CHI = {Proc. ACM Conf. on Human Factors in Computing Systems (CHI)}}
@STRING{CGF = {Computer Graphics Forum}}
@STRING{CGF_EG = {Computer Graphics Forum (Proc. Eurographics)}}
@STRING{CGF_SGP = {Computer Graphics Forum (Proc. SGP)}}
@STRING{CRV = {Proc. Canadian Conf. on Computer \& Robot Vision}}
@STRING{CVPR = {Proc. IEEE Conf. on Computer Vision \& Pattern Recognition (CVPR)}}
@STRING{INFOVIS = {Proc. IEEE Information Visualization Symp. (INFOVIS)}}
@STRING{VAST = {Proc. IEEE Symp. on Visual Analytics Science \& Technology}}
@STRING{VASTC = {Proc. IEEE Conf. on Visual Analytics Science \& Technology (VAST)}}
@STRING{PVIS =  {Proc. IEEE Pacific Visualization Symp. (PacificVis)}}
@STRING{ECCV = {Proc. Euro. Conf. on Comp. Vis. (ECCV)}}
@STRING{FGR = {Proc. IEEE Conf. on Automatic Face \& Gesture Recognition}}
@STRING{ICIP = {Proc. IEEE Conf. on Image Processing (ICIP)}}
@STRING{ICASSP = {Proc. Int. Conf. on Acoustics, Speech \& Signal Processing (ICASSP)}}
@STRING{ICCV = {Proc. Int. Conf. on Computer Vision (ICCV)}}
@STRING{LDAV = {Proc. IEEE Symp. on Large-Scale Data Analysis \& Visualization (LDAV)}}
@STRING{ICPR = {Proc. Int. Conf. on Pattern Recognition (ICPR)}}
@STRING{IJCV = {Int. Journal of Computer Vision}}
@STRING{PAMI = {IEEE Trans. Pattern Analysis \& Machine Intelligence}}
@STRING{SGP = {Symp. on Geom. Proc.}}
@STRING{SIGGRAPH = {Proc. of SIGGRAPH}}
@STRING{SMI = {Proc. IEEE Int. Conf. on Shape Modeling \& Applications}}
@STRING{TOG = {ACM Trans. on Graphics}}
@STRING{TVC = {Visual Computer}}
@STRING{TVCG = {IEEE Trans. on Visualization \& Computer Graphics}}
@STRING{SIG_TOG = {ACM Trans. on Graphics (Proc. SIGGRAPH)}}
@STRING{SIGA_TOG = {ACM Trans. on Graphics (Proc. SIGGRAPH Asia)}}
@STRING{SIGGRAPH = {Proc. SIGGRAPH}}
@STRING{SIGMOD = {Proc. ACM Int. Conf. on Management of Data (SIGMOD)}}
@STRING{ICML = {Proc. Int. Conf. on Machine Learning (ICML)}}
@STRING{NIPS = {Advances in Neural Information Processing Systems (NIPS)}}
@STRING{PR = {Pattern Recognition}}
@STRING{IV = {Proc. Int. Conf. on Information Visualization (IV)}}
@STRING{IVJ = {Information Visualization}}
@STRING{ITIT = {it - Information Technology}}
@STRING{JASA = {Journal of the American Statistical Association}}
@STRING{COGSCI = {Proc. Annual Meeting of the Cognitive Science Society (CogSci)}}
@STRING{JCGS = {Journal of Computational \& Graphical Statistics}}
@STRING{JMLR = {Journal of Machine Learning Research (JMLR)}}
@STRING{ISSG = {Proc. Int. Symp. Smart Graphics}}
@STRING{KDD = {Proc. Int. Conf. on Knowledge Discovery and Data Mining (KDD)}}
@STRING{TKDD = {ACM Trans. on Knowledge Discovery from Data}} 
@STRING{TNN={IEEE Trans. on Neural Networks}}
@STRING{TOC={IEEE Trans. on Computers}}
@STRING{CSDA={Computational Statistics and Data Analysis}}


@ARTICLE{ScatterNet_Ma2018, 
author={Y. {Ma} and A. K. H. {Tung} and W. {Wang} and X. {Gao} and Z. {Pan} and W. {Chen}}, 
journal={IEEE Transactions on Visualization and Computer Graphics}, 
title={ScatterNet: A Deep Subjective Similarity Model for Visual Analysis of Scatterplots}, 
year={2018}, 
pages={1-1}, 
doi={10.1109/TVCG.2018.2875702}, 
ISSN={1077-2626}, 
}


@article{ClustMe_eurovis2019,
  author = {Mostafa M. Abbas and Micha{\"{e}}l Aupetit and Michael Sedlmair and Halima Bensmail},
  journal = {Computer Graphics Forum},
  title = {ClustMe: A Visual Quality Measure for Ranking Monochrome Scatterplots based on Cluster Patterns.},
  year = 2019,
  doi = {10.1111/cgf.13684},
}

@inproceedings{Tukey1985,
    author = {J. W. Tukey  and P. A. Tukey},
    booktitle = {Proc. the Sixth Annual Conference and Exposition: Computer Graphics, Vol. III, Technical Sessions},
    organization = {Nat. Computer Graphics Association},
    pages = {773--785},
    title = {{Computer Graphics and Exploratory Data Analysis: An Introduction}},
    year = {1985}
}

@article{Rpackagecaret,
    title = {caret: Classification and Regression Training},
    author = {Max Kuhn},
    year = {2019},
    journal = {R package version 6.0-82},
    url = {https://CRAN.R-project.org/package=caret},
  }
  
@article{KinVisSoftware_Ullah2019,
  author    = {Ehsan Ullah and
               Micha{\"{e}}l Aupetit and
               Arun Das and
               Abhishek Patil and
               Nooral Al Muftah and
               Reda Rawi and
               Mohamad Saad and
               Halima Bensmail},
  title     = {KinVis: a visualization tool to detect cryptic relatedness in genetic
               datasets},
  journal   = {Bioinform.},
  volume    = {35},
  number    = {15},
  pages     = {2683--2685},
  year      = {2019},
  doi       = {10.1093/bioinformatics/bty1028},
}


@Article{Auton2015,
  author    = {Adam Auton and others},
  title     = {A global reference for human genetic variation},
  journal   = {Nature},
  year      = {2015},
  volume    = {526},
  number    = {7571},
  pages     = {68--74},
  publisher = {Nature Publishing Group},
}

@Article{Elhaik2022,
author={Eran Elhaik},
title={Principal Component Analyses (PCA)-based findings in population genetic studies are highly biased and must be reevaluated},
journal={Scientific Reports},
year={2022},
month={Aug},
day={29},
volume={12},
number={1},
pages={14683},
abstract={Principal Component Analysis (PCA) is a multivariate analysis that reduces the complexity of datasets while preserving data covariance. The outcome can be visualized on colorful scatterplots, ideally with only a minimal loss of information. PCA applications, implemented in well-cited packages like EIGENSOFT and PLINK, are extensively used as the foremost analyses in population genetics and related fields (e.g., animal and plant or medical genetics). PCA outcomes are used to shape study design, identify, and characterize individuals and populations, and draw historical and ethnobiological conclusions on origins, evolution, dispersion, and relatedness. The replicability crisis in science has prompted us to evaluate whether PCA results are reliable, robust, and replicable. We analyzed twelve common test cases using an intuitive color-based model alongside human population data. We demonstrate that PCA results can be artifacts of the data and can be easily manipulated to generate desired outcomes. PCA adjustment also yielded unfavorable outcomes in association studies. PCA results may not be reliable, robust, or replicable as the field assumes. Our findings raise concerns about the validity of results reported in the population genetics literature and related fields that place a disproportionate reliance upon PCA outcomes and the insights derived from them. We conclude that PCA may have a biasing role in genetic investigations and that 32,000-216,000 genetic studies should be reevaluated. An alternative mixed-admixture population genetic model is discussed.},
issn={2045-2322},
doi={10.1038/s41598-022-14395-4},
}


@article{Quadri2022,
  author       = {Ghulam Jilani Quadri and
                  Jennifer Adorno Nieves and
                  Brenton M. Wiernik and
                  Paul Rosen},
  title        = {Automatic Scatterplot Design Optimization for Clustering Identification},
  journal      = {{IEEE} Trans. Vis. Comput. Graph.},
  volume       = {29},
  number       = {10},
  pages        = {4312--4327},
  year         = {2023},
  doi          = {10.1109/TVCG.2022.3189883},
}

@ARTICLE{Quadri2021,
  author={Ghulam Jilani Quadri and  Paul Rosen},
  journal={IEEE Transactions on Visualization and Computer Graphics}, 
  title={Modeling the Influence of Visual Density on Cluster Perception in Scatterplots Using Topology}, 
  year={2021},
  volume={27},
  number={2},
  pages={1829-1839},
  doi={10.1109/TVCG.2020.3030365}}
  
@inproceedings{KinVisPvis_Aupetit2016,
  author    = {Micha{\"{e}}l Aupetit and
               Ehsan Ullah and
               Reda Rawi and
               Halima Bensmail},
  editor    = {Chuck Hansen and
               Ivan Viola and
               Xiaoru Yuan},
  title     = {A design study to identify inconsistencies in kinship information:
               The case of the 1000 Genomes project},
  booktitle = {2016 {IEEE} Pacific Visualization Symposium, PacificVis 2016, Taipei,
               Taiwan, April 19-22, 2016},
  pages     = {254--258},
  publisher = {{IEEE} Computer Society},
  year      = {2016},
  doi       = {10.1109/PACIFICVIS.2016.7465281},

}


  
  @article{Feng_2020, 
  title={Dimension Reduction and Clustering Models for Single-Cell RNA Sequencing Data: A Comparative Study}, volume={21}, ISSN={1422-0067}, 
  DOI={10.3390/ijms21062181}, number={6}, journal={International Journal of Molecular Sciences}, 
  publisher={MDPI AG}, 
  author={Feng, Chao and Liu, Shufen and Zhang, Hao and Guan, Renchu and Li, Dan and Zhou, Fengfeng and Liang, Yanchun and Feng, Xiaoyue}, 
  year={2020}, month={Mar}, pages={2181}
  }
  
  @inproceedings{PerceptionBasedClustering_AupetitSABB19,
  author    = {Micha{\"{e}}l Aupetit and
               Michael Sedlmair and
               Mostafa M. Abbas and
               Abdelkader Baggag and
               Halima Bensmail},
  title     = {Toward Perception-Based Evaluation of Clustering Techniques for Visual
               Analytics},
  booktitle = {2019 {IEEE} Visualization Conference, {VIS} 2019, Vancouver, BC, Canada,
               October 20-25, 2019},
  pages     = {141--145},
  publisher = {{IEEE}},
  year      = {2019},
  doi       = {10.1109/VISUAL.2019.8933620},
}
  
  @Article{Han2017,
author={Z. Han and T. Johnson and J. Zhang and X. Zhang and K. Huang},
title={Functional Virtual Flow Cytometry: A Visual Analytic Approach for Characterizing Single-Cell Gene Expression Patterns},
journal={BioMed research international},
year={2017},
edition={2017/07/17},
publisher={Hindawi},
volume={2017},
pages={3035481-3035481},
abstract={We presented a novel workflow for detecting distribution patterns in cell populations based on single-cell transcriptome study. With the fast adoption of single-cell analysis, a challenge to researchers is how to effectively extract gene features to meaningfully separate the cell population. Considering that coexpressed genes are often functionally or structurally related and the number of coexpressed modules is much smaller than the number of genes, our workflow uses gene coexpression modules as features instead of individual genes. Thus, when the coexpressed modules are summarized into eigengenes, not only can we interactively explore the distribution of cells but also we can promptly interpret the gene features. The interactive visualization is aided by a novel application of spatial statistical analysis to the scatter plots using a clustering index parameter. This parameter helps to highlight interesting 2D patterns in the scatter plot matrix (SPLOM). We demonstrated the effectiveness of the workflow using two large single-cell studies. In the Allen Brain scRNA-seq dataset, the visual analytics suggested a new hypothesis such as the involvement of glutamate metabolism in the separation of the brain cells. In a large glioblastoma study, a sample with a unique cell migration related signature was identified.},
issn={2314-6141},
doi={10.1155/2017/3035481},
}


  
  @Article{Kiselev2019,
author={V. Y. Kiselev and T. S. Andrews and M. Hemberg},
title={Challenges in unsupervised clustering of single-cell RNA-seq data},
journal={Nature Reviews Genetics},
year={2019},
month={May},
day={01},
volume={20},
number={5},
pages={273-282},
abstract={Single-cell RNA sequencing (scRNA-seq) allows researchers to collect large catalogues detailing the transcriptomes of individual cells. Unsupervised clustering is of central importance for the analysis of these data, as it is used to identify putative cell types. However, there are many challenges involved. We discuss why clustering is a challenging problem from a computational point of view and what aspects of the data make it challenging. We also consider the difficulties related to the biological interpretation and annotation of the identified clusters.},
issn={1471-0064},
doi={10.1038/s41576-018-0088-9},
}


 @ARTICLE{MCC_Boughorbel2017,
       author = {S. {Boughorbel} and F. {Jarray} and M. {El-Anbari}},
        title = "{Optimal classifier for imbalanced data using Matthews Correlation Coefficient metric}",
      journal = {PLoS ONE},
         year = 2017,
        month = jun,
       volume = {12},
       number = {6},
        pages = {e0177678},
          doi = {10.1371/journal.pone.0177678},
}

@article{CARET_Kuhn2008,
   author = {Max Kuhn},
   title = {Building Predictive Models in R Using the caret Package},
   journal = {Journal of Statistical Software},
   volume = {28},
   number = {5},
   year = {2008},
   issn = {1548-7660},
   pages = {1--26},
   doi = {10.18637/jss.v028.i05},
}


@article{ROSE_Menardi2014,
author = {G. Menardi and N. Torelli},
year = {2014},
title = {Training and assessing classification rules with imbalanced data},
journal = {Data Mining and Knowledge Discovery}, 
volume = 28,
pages = {92--122},
}

@article{SMOTE_Chawla2002,
author = {N. V. Chawla and K. W. Bowyer and L. O. Hall and W. P. Kegelmeyer},
year = {2002},
title = {Smote: Synthetic minority over-sampling technique},
journal = {Journal of Artificial Intelligence Research}, 
volume = 16,
pages = {321--357},
}


@ARTICLE{SupDRSepMe_Wang2018,  
author={Y. {Wang} and K. {Feng} and X. {Chu} and J. {Zhang} and C. {Fu} and M. {Sedlmair} and X. {Yu} and B. {Chen}},  journal={IEEE Transactions on Visualization and Computer Graphics},  title={A Perception-Driven Approach to Supervised Dimensionality Reduction for Visualization},   year={2018},  volume={24},  number={5},  pages={1828-1840},}

@ARTICLE{OptimColorSepMe_Wang2019, 
author={Y. {Wang} and X. {Chen} and T. {Ge} and C. {Bao} and M. {Sedlmair} and C. {Fu} and O. {Deussen} and B. {Chen}}, journal={IEEE Transactions on Visualization and Computer Graphics}, title={Optimizing Color Assignment for Perception of Class Separability in Multiclass Scatterplots}, year={2019}, volume={25}, number={1}, pages={820-829},
}

@ARTICLE{DimRedClustVA_Wenskovitch2018,
author={J. {Wenskovitch} and I. {Crandell} and N. {Ramakrishnan} and L. {House} and S. {Leman} and C. {North}},
journal={IEEE Transactions on Visualization and Computer Graphics},
title={Towards a Systematic Combination of Dimension Reduction and Clustering in Visual Analytics},
year={2018},
volume={24},
number={1},
pages={131-141},
doi={10.1109/TVCG.2017.2745258},
ISSN={2160-9306},
month={Jan},}

@INPROCEEDINGS{RadViz_Hoffman1999,
    author = {Patrick Hoffman and Georges Grinstein and David Pinkney},
    title = {Dimensional anchors: A graphic primitive for multidimensional multivariate information visualizations},
    booktitle = {In Proc of the NPIV 99},
    year = {1999},
    pages = {9--16},
    publisher = {ACM Press}
}
@ARTICLE{RadVizVsStarCoord_Rubio2016,
author={M. {Rubio-Sánchez} and L. {Raya} and F. {Díaz} and A. {Sanchez}},
journal={IEEE Transactions on Visualization and Computer Graphics},
title={A comparative study between RadViz and Star Coordinates},
year={2016},
volume={22},
number={1},
pages={619-628},
doi={10.1109/TVCG.2015.2467324},
ISSN={2160-9306},
month={Jan},}

@ARTICLE{Clustrophile2_Cavallo2019,
author={M. {Cavallo} and C. {Demiralp}},
journal={IEEE Transactions on Visualization and Computer Graphics},
title={Clustrophile 2: Guided Visual Clustering Analysis},
year={2019},
volume={25},
number={1},
pages={267-276},
doi={10.1109/TVCG.2018.2864477},
ISSN={2160-9306},
month={Jan},}

@ARTICLE{Brehmer13_MultiLevelTaskTypology, 
author={M. {Brehmer} and T. {Munzner}}, 
journal=TVCG, 
title={A Multi-Level Typology of Abstract Visualization Tasks}, 
year={2013}, 
volume={19}, 
number={12}, 
pages={2376-2385}, 
doi={10.1109/TVCG.2013.124}, 
ISSN={1077-2626}, 
}

@INPROCEEDINGS{Albuquerque11_PerceptionBasedVQM, 
author={G. {Albuquerque} and M. {Eisemann} and M. {Magnor}}, 
booktitle=VAST, 
title={Perception-based visual quality measures}, 
year={2011}, 
pages={13-20}, 
doi={10.1109/VAST.2011.6102437}, 
}



@INPROCEEDINGS{Mcgrath95methodologymatters,
    author = {E. Mcgrath},
    title = {Methodology matters: Doing research in the behavioral and social sciences},
    booktitle = {Readings in Human-Computer Interaction: Toward the Year 2000 (2nd. eds.)},
    year = {1995},
    pages = {152--169},
    publisher = {Morgan Kaufman}
}

@inproceedings{SchulzNEFHHKNSB16,
  author    = {Christoph Schulz and
               Arlind Nocaj and
               Mennatallah El{-}Assady and
               Steffen Frey and
               Marcel Hlawatsch and
               Michael Hund and
               Grzegorz Karol Karch and
               Rudolf Netzel and
               Christin Sch{\"{a}}tzle and
               Miriam Butt and
               Daniel A. Keim and
               Thomas Ertl and
               Ulrik Brandes and
               Daniel Weiskopf},
  title     = {Generative Data Models for Validation and Evaluation of Visualization
               Techniques},
  booktitle = BELIV,
  pages     = {112--124},
  year      = {2016},
  doi       = {10.1145/2993901.2993907}
}

@article{BehrischBKSEFSD18,
  author    = {Michael Behrisch and
               Michael Blumenschein and
               Nam Wook Kim and
               Lin Shao and
               Mennatallah El{-}Assady and
               Johannes Fuchs and
               Daniel Seebacher and
               Alexandra Diehl and
               Ulrik Brandes and
               Hanspeter Pfister and
               Tobias Schreck and
               Daniel Weiskopf and
               Daniel A. Keim},
  title     = {Quality Metrics for Information Visualization},
  journal   = CGF,
  volume    = {37},
  number    = {3},
  pages     = {625--662},
  year      = {2018},
  url       = {https://doi.org/10.1111/cgf.13446},
  doi       = {10.1111/cgf.13446}
}


@Article{Isenberg:2017:VMC,
  author = {Petra Isenberg and Florian Heimerl and Steffen Koch and Tobias Isenberg and Panpan Xu and Chad Stolper and Michael Sedlmair and Jian Chen and Torsten M{\"o}ller and John Stasko},
	title = {{vispubdata.org: A Metadata Collection about {IEEE} Visualization ({VIS}) Publications}},
	journal = TVCG,
	year = {2017},
	volume = {23},
	doi = {10.1109/TVCG.2016.2615308},
}

@inproceedings{kmeans_macqueen1966,
  author = {J. MacQueen},
  booktitle = {Berkeley Symposium on Mathematical Statistics and Probability},
  title = {Some Methods for Classification and Analysis of Multivariate Observations},
  year = 1966
}


@inproceedings{iPCA_Jeong2009,
author = {Dong Hyun Jeong and Caroline Ziemkiewicz and Brian Fisher  and William Ribarsky mand Remco Chang},
title = {IPCA: An Interactive System for PCA-Based Visual Analytics},
year = {2009},
publisher = {The Eurographs Association \& John Wiley \& Sons, Ltd.},
address = {Chichester, GBR},
doi = {10.1111/j.1467-8659.2009.01475.x},
booktitle = {Proceedings of the 11th Eurographics / IEEE - VGTC Conference on Visualization},
pages = {767–774},
numpages = {8},
location = {Berlin, Germany},
series = {EuroVis’09}
}


@book{Ware:2004:IVP,
  author = {Colin Ware},
  title = {Information Visualization: Perception for Design},
  edition = {2\textsuperscript{nd}},
  year = 2004,
  publisher = {Morgan Kaufmann Publishers Inc.},
  address = {San Francisco},
	doi = {10.1016/B978-155860819-1/50001-7}
}

########################################
@inproceedings{Wilkinson_scagnostics2005,
  author = {Leland Wilkinson and Anushka Anand and Robert L. Grossman},
  booktitle = INFOVIS,
  editor = {Stasko, John T. and Ward, Matthew O.},
  doi = {10.1109/INFOVIS.2005.14},
  isbn = {0-7803-9464-X},
  pages = 21,
  publisher = {IEEE Computer Society},
  title = {Graph-Theoretic Scagnostics.},
  year = 2005
}

@ARTICLE{Matute2018_skeletonScagnostics, 
author={J. Matute and A. C. Telea and L. Linsen}, 
journal=TVCG, 
title={Skeleton-Based Scagnostics}, 
year={2018}, 
volume={24}, 
number={1}, 
pages={542-552}, 
doi={10.1109/TVCG.2017.2744339}, 
ISSN={1077-2626}, 
}


@ARTICLE{Johansson_clustqualmetric2009, 
author={S. Johansson and J. Johansson}, 
journal=TVCG, 
title={Interactive Dimensionality Reduction Through User-defined Combinations of Quality Metrics}, 
year={2009}, 
volume={15}, 
number={6}, 
pages={993-1000}, 
doi={10.1109/TVCG.2009.153}, 
ISSN={1077-2626}, 
}

@inproceedings{agrawal1998automaticClustering,
  author = {R. Agrawal and J. Gehrke and D. Gunopulos and P. Raghavan},
  booktitle = SIGMOD,
  keywords = {clique clustering data dimensional high lecture:2014 lecture:2016 lecture:data-mining subspace},
  pages = {94--105},
  publisher = {ACM Press},
  title = {Automatic Subspace Clustering of High Dimensional Data for Data Mining Applications},
  year = 1998
}

@article{ImgDataAugment_Shorten2019,
  author = {Connor Shorten and Taghi M. Khoshgoftaar},
  ee = {https://doi.org/10.1186/s40537-019-0197-0},
  journal = {J. Big Data},
  pages = 60,
  title = {A survey on Image Data Augmentation for Deep Learning.},
  volume = 6,
  year = 2019
}


@inproceedings{BIRCH_zhang1996,
  address = {New York, NY, USA},
  author = {Tian Zhang and Raghu Ramakrishnan and Miron Livny},
  booktitle = SIGMOD,
  isbn = {0-89791-794-4},
  location = {Montreal, Quebec, Canada},
  numpages = {12},
  pages = {103--114},
  title = {BIRCH: An Efficient Data Clustering Method for Very Large Databases},
  doi = {10.1145/233269.233324},
  year = 1996
}
@inproceedings{CURE_GuhaRS98,
  author = {Sudipto Guha and Rajeev Rastogi and Kyuseok Shim},
  booktitle = SIGMOD,
  editor = {Haas, Laura M. and Tiwary, Ashutosh},
  doi = {10.1145/276304.276312},
  isbn = {0-89791-995-5},
  pages = {73-84},
  title = {CURE: An Efficient Clustering Algorithm for Large Databases.},
  year = 1998
}

@inproceedings{FeldmanFK11,
  author = {Dan Feldman and Matthew Faulkner and Andreas Krause},
  booktitle = NIPS,
  editor = {Shawe-Taylor, John and Zemel, Richard S. and Bartlett, Peter L. and Pereira, Fernando C. N. and Weinberger, Kilian Q.},
  ee = {http://papers.nips.cc/paper/4363-scalable-training-of-mixture-models-via-coresets},
  pages = {2142-2150},
  title = {Scalable Training of Mixture Models via Coresets.},
  year = 2011
}

@inproceedings{GanT15,
  author = {Junhao Gan and Yufei Tao},
  booktitle = SIGMOD,
  editor = {Sellis, Timos K. and Davidson, Susan B. and Ives, Zachary G.},
  doi = {10.1145/2723372.2737792},
  isbn = {978-1-4503-2758-9},
  pages = {519-530},
  title = {DBSCAN Revisited: Mis-Claim, Un-Fixability, and Approximation.},
  year = 2015
}


@article{fraley200201,
  author = {Chris Fraley and Adrian E. Raftery},
  journal = JASA,
  pages = {611-631},
  title = {Model-Based Clustering, Discriminant Analysis and Density Estimation},
  volume = 97,
  year = 2002
}



@Article{CorrelScatterplots_Rensink2017,
author="Ronald A. Rensink",
title="The nature of correlation perception in scatterplots",
journal="Psychonomic Bulletin {\&} Review",
year="2017",
day="01",
volume="24",
number="3",
pages="776--797",
issn="1531-5320",
doi="10.3758/s13423-016-1174-7",
}

@article{PerceptSegmentDotClusters_Cohen2008,
author = {Elias H. Cohen and Manish Singh and Laurence T. Maloney},
title = {Perceptual segmentation and the perceived orientation
of dot clusters: The role of robust statistics},
journal = {Journal of Vision},
volume = {8},
number = {7},
pages = {6},
year = {2008},
doi = {10.1167/8.7.6},
}

@article{Callaghan74,
author = {J. F. O'Callaghan},
title ={Human Perception of Homogeneous Dot Patterns},
journal = {Perception},
volume = {3},
number = {1},
pages = {33-45},
year = {1974},
doi = {10.1068/p030033},
}

@article{AnobileNumerosity2016,
author = {Giovanni Anobile and Guido Marco Cicchini and David C. Burr},
title ={Number As a Primary Perceptual Attribute: A Review},
journal = {Perception},
volume = {45},
number = {1-2},
pages = {5-31},
year = {2016},
doi = {10.1177/0301006615602599},
}


@article{Coh60,
  author = {J. Cohen},
  journal = {Educational and Psychological Measurement},
  pages = {37--46},
  title = {A coefficient of agreement for nominal scales},
  volume = 20,
  year = 1960
}



@article{landis1977measurement,
  author = {J. Richard Landis and Gary G. Koch},
  journal = {Biometrics},
  pages = {159--174},
  publisher = {JSTOR},
  title = {The measurement of observer agreement for categorical data},
  year = 1977
}


@article {KappaExpValueMcHugh2012,
author = {Marry L. McHugh},
title = {Interrater reliability: the kappa statistic},
volume = {22},
number = {3},
pages = {276-282},
year = {2012},
doi = {10.11613/BM.2012.031},
publisher = {Biochemia Medica},
issn = {1330-0962},
journal = {Biochem Med (Zagreb)}
}



@article{PerceptOfAvgVal_Gleicher2013,
  author = {Michael Gleicher and Michael Correll and Christine Nothelfer and Steven Franconeri},
  doi = {10.1109/TVCG.2013.183},
  journal = TVCG,
  number = 12,
  pages = {2316-2325},
  title = {Perception of Average Value in Multiclass Scatterplots.},
  volume = 19,
  year = 2013
}



@article{ClusterPerception_Sadahiro1997,
author = {Yukio Sadahiro},
title = {Cluster Perception in the Distribution of Point Objects},
journal = {Cartographica: The International Journal for Geographic Information and Geovisualization},
volume = {34},
number = {1},
pages = {49-62},
year = {1997},
doi = {10.3138/Y308-2422-8615-1233},
}


@article{VanbelleKappa_2009,
author = {S. Vanbelle and A. Albert},
title = {Agreement between an isolated rater and a group of raters},
journal = {Statistica Neerlandica},
volume = {63},
number = {1},
pages = {82-100},
year = 2009,
doi = {10.1111/j.1467-9574.2008.00412.x},
}

@ARTICLE{MDPsurveyNonatoAupetit2018, 
author={L. G. Nonato and M. Aupetit}, 
journal=TVCG, 
title={Multidimensional Projection for Visual Analytics: Linking Techniques with Distortions, Tasks, and Layout Enrichment}, 
year={2018}, 
doi={10.1109/TVCG.2018.2846735}, 
ISSN={1077-2626}, 
}

@article{BensmailC1996,
 ISSN = {01621459},
 URL = {http://www.jstor.org/stable/2291604},
 author = {Halima Bensmail and Gilles Celeux},
 journal = JASA,
 number = {436},
 pages = {1743--1748},
 publisher = {[American Statistical Association, Taylor & Francis, Ltd.]},
 title = {Regularized Gaussian Discriminant Analysis Through Eigenvalue Decomposition},
 volume = {91},
 year = {1996}
}


@article{Bensmail1997,
author = {H. Bensmail and G. Celeux and A.E. Raftery and C. Robert},
title={Inference in model-based cluster analysis},
journal = {Statistics and Computing}, 
volume =7, 
pages = {1-10},
year=1997
}

@article{schwarz78_BIC,
  author = {G. Schwarz},
  journal = {The annals of statistics},
  pages = {461-464},
  title = {Estimating the dimension of a model},
  volume = 6,
  year = 1978
}


@article{Bouveyron2014,
 author = {Charles Bouveyron and Camille Brunet-Saumard},
 title = {Model-based Clustering of High-dimensional Data: A Review},
 journal = CSDA, 
 issue_date = {March, 2014},
 volume = {71},
 year = {2014},
 issn = {0167-9473},
 pages = {52--78},
 numpages = {27},
 doi = {10.1016/j.csda.2012.12.008},
 publisher = {Elsevier Science Publishers B. V.},
 address = {Amsterdam, The Netherlands, The Netherlands},
} 

@article{DGaillardAG08,
  author    = {Pierre Gaillard and
               Micha{\"{e}}l Aupetit and
               G{\'{e}}rard Govaert},
  title     = {Learning topology of a labeled data set with the supervised generative Gaussian graph},
  journal   = {Neurocomputing},
  volume    = {71},
  number    = {7-9},
  pages     = {1283--1299},
  year      = {2008},
  doi       = {10.1016/j.neucom.2007.12.028},
}

@inproceedings{MaasHTBCH15,
  author = {Ryan Maas and Jeremy Hyrkas and Olivia Grace Telford and Magdalena Balazinska and Andrew J. Connolly and Bill Howe},
  booktitle = {Proc. of the 3rd VLDB Workshop on In-Memory Data Mangement and Analytics},
  doi = {10.1145/2803140.2803143},
  isbn = {978-1-4503-3713-7},
  pages = {3:1-3:8},
  publisher = {ACM},
  title = {Gaussian Mixture Models Use-Case: In-Memory Analysis with Myria.},
  year = 2015
}

@inproceedings{FastGMM_Moore1999,
 author = {Andrew W. Moore},
 title = {Very Fast EM-based Mixture Model Clustering Using Multiresolution Kd-trees},
 booktitle = NIPS,
 year = {1999},
 isbn = {0-262-11245-0},
 pages = {543--549},
 numpages = {7},
 publisher = {MIT Press},
} 

@article{BarnesHutTSNE_Maaten14,
  author = {van der Maaten, Laurens},
  journal = JMLR,
  number = 1,
  pages = {3221-3245},
  title = {Accelerating t-SNE using tree-based algorithms.},
  volume = 15,
  year = 2014
}



@article{Silhouettes_ROUSSEEUW1987,
title = "Silhouettes: A graphical aid to the interpretation and validation of cluster analysis",
journal = {Journal of Computational and Applied Mathematics},
volume = "20",
number = "Supplement C",
pages = "53 - 65",
year = "1987",
issn = "0377-0427",
doi = "10.1016/0377-0427(87)90125-7",
author = "Peter J. Rousseeuw",
}

@INPROCEEDINGS{OPTICS_Ankerst99,
    author = {Michael Ankerst and Markus M. Breunig and Hans-peter Kriegel and Jörg Sander},
    title = {OPTICS: Ordering Points To Identify the Clustering Structure},
    booktitle = SIGMOD,
    year = {1999},
    pages = {49--60},
    publisher = {ACM Press}
}

@article{JinWL05,
  author = {Huidong Jin and Man Leung Wong and Kwong-Sak Leung},
  doi = {10.1109/TPAMI.2005.226},
  journal = PAMI,
  number = 11,
  pages = {1710-1719},
  title = {Scalable Model-Based Clustering for Large Databases Based on Data Summarization.},
  volume = 27,
  year = 2005
}

@inproceedings{HumanComputation_Quinn2011,
 author = {Alexander J. Quinn and Benjamin B. Bederson},
 title = {Human Computation: A Survey and Taxonomy of a Growing Field},
 booktitle = CHI,
 year = {2011},
 isbn = {978-1-4503-0228-9},
 location = {Vancouver, BC, Canada},
 pages = {1403--1412},
 numpages = {10},
 doi = {10.1145/1978942.1979148},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@article{recaptcha_von2008,
  author = {Luis Von Ahn and Benjamin Maurer and Colin McMillen and David Abraham, and Manuel Blum},
  journal = {Science},
  number = 5895,
  pages = {1465--1468},
  publisher = {American Association for the Advancement of Science},
  title = {{reCAPTCHA}: Human-Based Character Recognition via Web Security Measures},
  volume = 321,
  year = 2008
}

@article{AIDR_Ofli2016,
author = {Ferda Ofli and Patrick Meier and Muhammad Imran and Carlos Castillo and Devis Tuia and Nicolas Rey and Julien Briant and Pauline Millet and Friedrich Reinhard and Matthew Parkan and Stéphane Joost},
title = {Combining Human Computing and Machine Learning to Make Sense of Big (Aerial) Data for Disaster Response},
journal = {Big Data},  
vol = 4,
number = 1,
pages = {47--59},
doi ={10.1089/big.2014.0064},
year = 2016
}

@article{ClusterSculptor_BRUNEAU2015,
title = "Cluster Sculptor, an interactive visual clustering system",
journal = "Neurocomputing",
volume = "150",
number = "Part B",
pages = "627 - 644",
year = "2015",
note = "Special Issue on Information Processing and Machine Learning for Applications of Engineering Solving Complex Machine Learning Problems with Ensemble Methods Visual Analytics using Multidimensional Projections",
issn = "0925-2312",
doi = "10.1016/j.neucom.2014.09.062",
author = "P. Bruneau and P. Pinheiro and B. Broeksema and B. Otjacques",
}

@article{Sepme1_SedlmairA15,
  author    = {Michael Sedlmair and
               Micha{\"{e}}l Aupetit},
  title     = {Data-driven Evaluation of Visual Quality Measures},
  journal   = CGF,
  volume    = {34},
  number    = {3},
  pages     = {201--210},
  year      = {2015},
  doi       = {10.1111/cgf.12632},
}

@article{RBFunivApprox_Park1991,
 author = {J. Park mand I. W. Sandberg},
 title = {Universal Approximation Using Radial-basis-function Networks},
 journal = {Neural Computation},
 volume = {3},
 number = {2},
 year = {1991},
 issn = {0899-7667},
 pages = {246--257},
 numpages = {12},
 doi = {10.1162/neco.1991.3.2.246},
 publisher = {MIT Press},
 address = {Cambridge, MA, USA},
} 

@article{Sepme2_AupetitS16,
  author    = {Micha{\"{e}}l Aupetit and
               Michael Sedlmair},
  title     = {SepMe: 2002 New visual separation measures},
  journal   = PVIS,
  pages     = {1--8},
  year      = {2016},
  doi       = {10.1109/PACIFICVIS.2016.7465244},
}

@article{taxonomySepme_SedlmairTMT12,
  author    = {Michael Sedlmair and
               A. Tatu and
               Tamara Munzner and
               Melanie Tory},
  title     = {A Taxonomy of Visual Cluster Separation Factors},
  journal   = CGF,
  volume    = {31},
  number    = {3},
  pages     = {1335--1344},
  year      = {2012},
  doi       = {10.1111/j.1467-8659.2012.03125.x},
}

@article{Sedlmair2013_ScatterplotAndDR,
  author = {Michael  Sedlmair and Tamara Munzner and Melanie Tory},
  doi = {10.1109/TVCG.2013.153},
  journal = TVCG,
  number = 12,
  pages = {2634-2643},
  title = {Empirical Guidance on Scatterplot and Dimension Reduction Technique Choices.},
  volume = 19,
  year = 2013
}



@inproceedings{subspaceclustering_TatuMFBSSK12,
  author    = {Andrada Tatu and
               Fabian Maass and
               Ines F{\"{a}}rber and
               Enrico Bertini and
               Tobias Schreck and
               Thomas Seidl and
               Daniel A. Keim},
  title     = {Subspace search and visualization to make sense of alternative clusterings
               in high-dimensional data},
  booktitle = VAST,
  pages     = {63--72},
  year      = {2012},
  doi       = {10.1109/VAST.2012.6400488},
}

@inproceedings{VisualClusterAnalysis_PandeyKFBB16,
  author    = {Anshul Vikram Pandey and
               Josua Krause and
               Cristian Felix and
               Jeremy Boy and
               Enrico Bertini},
  title     = {Towards Understanding Human Similarity Perception in the Analysis of Large Sets of Scatter Plots},
  booktitle = CHI,
  pages     = {3659--3669},
  year      = {2016},
  doi       = {10.1145/2858036.2858155},
}

@article{RensinkB10_perceptionOfCorrelationInSP,
  author = {Ronald A. Rensink, and Gideon Baldridge},
  doi = {10.1111/j.1467-8659.2009.01694.x},
  journal = CGF,
  number = 3,
  pages = {1203-1210},
  title = {The Perception of Correlation in Scatterplots.},
  volume = 29,
  year = 2010
}
@article{Li2010_perceptionOfCorrelationInSPandPCP,
  author = {Jing Li and Jean-Bernard Martens and Jarke J. van Wijk},
  doi = {10.1057/ivs.2008.13},
  journal = {Information Visualization},
  number = 1,
  pages = {13-30},
  title = {Judging correlation from scatterplots and parallel coordinate plots.},
  volume = 9,
  year = 2010
}
@article{HarrisonYFC14_rankingVisOfCorrelWeberLaw,
  author = {Lane Harrison and Fumeng Yang, and Steven Franconeri and Remco Chang},
  doi = {10.1109/TVCG.2014.2346979},
  journal = TVCG,
  number = 12,
  pages = {1943-1952},
  title = {Ranking Visualizations of Correlation Using Weber's Law.},
  volume = 20,
  year = 2014
}

@article{DemiralpBH14_learningPerceptualKernel,
  author = {Cagatay Demiralp and Michael S. Bernstein and Jeffrey Heer},
  doi = {10.1109/TVCG.2014.2346978},
  journal = TVCG,
  number = 12,
  pages = {1933-1942},
  title = {Learning Perceptual Kernels for Visualization Design.},
  volume = 20,
  year = 2014
}

@inproceedings{TatuBBKS10,
  author = {Andrada Tatu and Peter Bak and Enrico Bertini and Daniel A. Keim and Jörn Schneidewind},
  booktitle = AVI,
  editor = {Giuseppe Santucci},
  doi = {10.1145/1842993.1843002},
  isbn = {978-1-4503-0076-6},
  pages = {49-56},
  publisher = {ACM Press},
  title = {Visual quality metrics and human perception: an initial study on 2D projections of large multidimensional data.},
  year = 2010
}

@article{EtemadpourMPMOL15,
  author = {Ronak Etemadpour and Robson Motta and Jose Gustavo de Souza Paiva and Rosane Minghim and Maria Cristina Ferreira de Oliveira and Lars Linsen},
  doi = {10.1109/TVCG.2014.2330617},
  journal = TVCG,
  number = 1,
  pages = {81-94},
  title = {Perception-Based Evaluation of Projection Methods for Multidimensional Data Visualization.},
  volume = 21,
  year = 2015
}

@article{primingAnchoringEffec_ValdezZS18,
  author = {André Calero Valdez and Martina Ziefle and Michael Sedlmair},
  doi = {10.1109/TVCG.2017.2744138},
  journal = TVCG,
  number = 1,
  pages = {584-594},
  title = {Priming and Anchoring Effects in Visualization.},
  volume = 24,
  year = 2018
}

@article{bekkar2013evaluation,
  title={Evaluation measures for models assessment over imbalanced datasets},
  author={Mohamed Bekkar and Hassiba Kheliouane Djemaa and Taklit Akrouf Alitouche},
  journal={Journal of Information Engineering and Applications},
  volume={3},
  number={10},
  year={2013}
}


@INPROCEEDINGS{DBSCAN_1996,
 author = {Martin Ester and Hans-Peter Kriegel and J\"{o}rg Sander and Xiaowei Xu},
 title = {A Density-based Algorithm for Discovering Clusters a Density-based Algorithm for Discovering Clusters in Large Spatial Databases with Noise},
 booktitle = KDD,
 year = {1996},
 location = {Portland, Oregon},
 pages = {226--231},
 numpages = {6},
 publisher = {AAAI Press},
} 


@INPROCEEDINGS{Pelleg00Xmeans,
    author = {Dau Pelleg and Andrew Moore},
    title = {X-means: Extending K-means with Efficient Estimation of the Number of Clusters},
    booktitle = ICML,
    year = {2000},
    pages = {727--734},
    publisher = {Morgan Kaufmann}
}


@ARTICLE{SubspaceVoyager_Wang2017,
author={B. {Wang} and K. {Mueller}},
journal={IEEE Transactions on Visualization and Computer Graphics},
title={The Subspace Voyager: Exploring High-Dimensional Data along a Continuum of Salient 3D Subspaces},
year={2018},
volume={24},
number={2},
pages={1204-1222},
doi={10.1109/TVCG.2017.2672987},
ISSN={2160-9306},
month={Feb},}

@ARTICLE{Buja2004TheoryOD,
  title={Theory of Dynamic Projections in High-Dimensional Data Visualization},
  author={Andreas Buja and Dianne Cook and Daniel Asimov and Catherine B. Hurley},
  year={2004},
  journal ="",
  url={https://api.semanticscholar.org/CorpusID:13001739}
}

@article{coclustering_govaert2013,
  title={Co-Clustering: Models, Algorithms and Applications},
  author={Gérard Govaert and Mohamed Nadif},
  journal={Wiley-ISTE},
  editor={ISBN 978-1-848-21473-6},
  pages = {256},
  year=2013
}

@inproceedings{Brehmer_BELIV14,
  author = {Matthew Brehmer and Michael Sedlmair and Stephen Ingram and Tamara Munzner},
  booktitle = BELIV,
  pages = {1-8},
  title = {Visualizing dimensionally-reduced data: interviews with analysts and a characterization of task sequences.},
  year = 2014
}


@article{imagequalitymetrics_LIN2011,
title = "Perceptual visual quality metrics: A survey",
journal = "Journal of Visual Communication and Image Representation",
volume = "22",
number = "4",
pages = "297 - 312",
year = "2011",
issn = "1047-3203",
doi = "10.1016/j.jvcir.2011.01.005",
author = "Weisi Lin and C.-C. Jay Kuo",
}

@inproceedings{VQM_BertiniS06,
  author    = {Enrico Bertini and
               Giuseppe Santucci},
  title     = {Visual quality metrics},
  booktitle = BELIV,
  pages     = {1--5},
  year      = {2006},
  doi       = {10.1145/1168149.1168159},
}

@ARTICLE{BeyondWeberLaw_Kay2016, 
author={M. Kay and J. Heer}, 
journal=TVCG, 
title={Beyond Weber's Law: A Second Look at Ranking Visualizations of Correlation}, 
year={2016}, 
volume={22}, 
number={1}, 
pages={469-478}, 
doi={10.1109/TVCG.2015.2467671}, 
ISSN={1077-2626}, 
}

@ARTICLE{qualMetric_Bertini11, 
author={E. Bertini and A. Tatu and D. Keim}, 
journal=TVCG, 
title={Quality Metrics in High-Dimensional Data Visualization: An Overview and Systematization}, 
year={2011}, 
volume={17}, 
number={12}, 
pages={2203-2212}, 
doi={10.1109/TVCG.2011.229}, 
ISSN={1077-2626}, 
}


@article{mergingGMM_Hennig10,
  author = {Christian Hennig},
  doi = {10.1007/s11634-010-0058-3},
  journal = {Advances in Data Analysis and Classification},
  number = 1,
  pages = {3-34},
  title = {Methods for merging Gaussian mixture components.},
  publisher = {Springer},
  volume = 4,
  year = 2010
}

@ARTICLE{SurveyClustering_Xu2005, 
author={Rui Xu and D. Wunsch}, 
journal=TNN, 
title={Survey of clustering algorithms}, 
year={2005}, 
volume={16}, 
number={3}, 
pages={645-678}, 
doi={10.1109/TNN.2005.845141}, 
ISSN={1045-9227}, 
}



@InProceedings{luxburg12a,
  title = 	 {Clustering: Science or Art?},
  author = 	 {Ulrike von Luxburg and Robert C. Williamson and Isabelle Guyon},
  booktitle = 	 {Proc. of ICML Workshop on Unsupervised and Transfer Learning},
  pages = 	 {65--79},
  year = 	 {2012},
  editor = 	 {Isabelle Guyon and Gideon Dror and Vincent Lemaire and Graham Taylor and Daniel Silver},
  volume = 	 {27},
  series = 	 {Proceedings of Machine Learning Research},
  address = 	 {Bellevue, Washington, USA},
  publisher = 	 {PMLR},
  url = 	 {http://proceedings.mlr.press/v27/luxburg12a.html},
}

@inproceedings{Aupetit14,
  author    = {Micha{\"{e}}l Aupetit},
  title     = {Sanity check for class-coloring-based evaluation of dimension reduction techniques},
  booktitle = BELIV,
  pages     = {134--141},
  year      = {2014},
  doi       = {10.1145/2669557.2669578},
}


@INPROCEEDINGS{scagexplorer_Wilkinson2014, 
author={T. N. Dang and L. Wilkinson}, 
booktitle=PVIS, 
title={ScagExplorer: Exploring Scatterplots by Their Scagnostics}, 
year={2014}, 
pages={73-80}, 
doi={10.1109/PacificVis.2014.42}, 
ISSN={2165-8765}, 
}


@article{rand1971,
  title={Objective criteria for the evaluation of clustering methods},
  author={William M. Rand},
  journal=JASA,
  volume={66},
  number={336},
  pages={846--850},
  year={1971},
  publisher={Taylor \& Francis Group}
}

@article{ray2005topography,
  title={The topography of multivariate normal mixtures},
  author={Surajit Ray and Bruce G. Lindsay},
  journal={Annals of Statistics},
  pages={2042--2065},
  year={2005},
  publisher={JSTOR}
}

@article{bhattacharyya1943measure,
  title={On a measure of divergence between two statistical populations defined by their probability distribution},
  author={Anil Bhattacharyya},
  journal={Bull. of Calcutta Mathematical Society},
  year={1943}
}


@article{hartigan1985dip,
  title={The dip test of unimodality},
  author={John A. Hartigan and Pamela M. Hartigan},
  journal={Annals of Statistics},
  pages={70--84},
  year={1985},
  publisher={JSTOR}
}

@inproceedings{tantrum2003assessment,
  title={Assessment and pruning of hierarchical model based clustering},
  author={Jeremy Tantrum and Alejandro Murua and Werner Stuetzle},
  booktitle=KDD,
  pages={197--205},
  year={2003},
}

@article{vinh2010information,
  title={Information theoretic measures for clusterings comparison: Variants, properties, normalization and correction for chance},
  author={Nguyen Xuan Vinh and Julien Epps and James Bailey},
  journal=JMLR,
  volume={11},
  pages={2837--2854},
  year={2010}
}

@article{LDA2005,
title = {Discriminant Analysis and Statistical Pattern Recognition},
author = {Geoffrey J. McLachlan},
publisher = {John Wiley & Sons, Inc.},
isbn = {9780471725299},
doi = {10.1002/0471725293.ch1},
pages = {1--26},
year = {2005}
}

@inproceedings{pelleg2000x,
  title={X-means: Extending K-means with Efficient Estimation of the Number of Clusters.},
  author={Dan Pelleg and Andrew W. Moore},
  booktitle=ICML,
  volume={1},
  pages={727--734},
  year={2000}
}

@article{gionis2007clustering,
  title={Clustering aggregation},
  author={Aristides Gionis and Heikki Mannila and Panayiotis Tsaparas},
  journal=TKDD,
  volume={1},
  number={1},
  pages={4},
  year={2007},
  publisher={ACM}
}

@article{nene1996columbia,
  title={Columbia object image library (coil-20)},
  author={Sameer A. Nene and Shree K. Nayar and Hiroshi Murase and others},
  year={1996},
  publisher={Technical report CUCS-005-96}
}

@article{veenman2002maximum,
  title={A maximum variance cluster algorithm},
  author={Cor J. Veenman and Marcel J. T. Reinders and Eric Backer},
  journal=PAMI,
  volume={24},
  number={9},
  pages={1273--1280},
  year={2002},
}

@article{fu2007flame,
  title={FLAME, a novel fuzzy clustering method for the analysis of DNA microarray data},
  author={Limin Fu and Enzo Medico},
  journal={BMC Bioinformatics},
  volume={8},
  number={1},
  pages={3},
  year={2007},
  publisher={BioMed Central}
}


@article{chang2008robust,
  title={Robust path-based spectral clustering},
  author={Hong Chang and Dit-Yan Yeung},
  journal={Pattern Recognition},
  volume={41},
  number={1},
  pages={191--203},
  year={2008},
  publisher={Elsevier}
}



@article{HopcroftT73_connectedComp,
  author = {John E. Hopcroft and Robert Endre Tarjan},
  doi = {10.1145/362248.362272},
  journal = {Commun. ACM},
  number = 6,
  pages = {372-378},
  title = {Efficient Algorithms for Graph Manipulation [H] (Algorithm 447).},
 volume = 16,
  year = 1973
}

@book{Palmer1999_VisionScience,
  author = {S.E. Palmer},
  publisher = {MIT Press},
  title = {Vision Science: Photons to Phenomenology},
  year = {1999}
}

@book{Dickinson2013_shapePerception,
author ={S. Dickinson and Z. Pizlo},
title={Shape Perception in Human and Computer Vision: An Interdisciplinary Perspective},
publisher = {Advances in Computer Vision and Pattern Recognition Series,Springer Verlag},
year = 2013,
}

@article{PALMER2003_groupingGestalt,
title = "When does grouping happen?",
journal = "Acta Psychologica",
volume = "114",
number = "3",
pages = "311 - 330",
year = "2003",
note = "Visual Gestalt Formation",
issn = "0001-6918",
doi = "10.1016/j.actpsy.2003.06.003",
author = "Stephen E. Palmer and Joseph L. Brooks and Rolf Nelson",
}

@book{sarndal2003model,
  title={Model assisted survey sampling},
  author={Carl-Erik S{\"a}rndal and Bengt Swensson and Jan Wretman},
  year={2003},
  publisher={Springer Science \& Business Media}
}

@article{dice1945measures,
  title={Measures of the amount of ecologic association between species},
  author={Lee R. Dice},
  journal={Ecology},
  volume={26},
  number={3},
  pages={297--302},
  year={1945},
  publisher={Wiley Online Library}
}

@article{price2010,
  title={New approaches to population stratification in genome-wide association studies},
  author={Alkes L. Price and Noah A. Zaitlen and David Reich and Nick Patterson},
  journal={Nature Reviews Genetics},
  volume={11},
  number={7},
  pages={459},
  year={2010},
  publisher={Nature Publishing Group}
}

@article{1000genomes,
  title={A global reference for human genetic variation},
  author={Genomes Project Consortium},
  journal={Nature},
  volume={526},
  number={7571},
  pages={68},
  year={2015},
  publisher={Nature Publishing Group}
}

@book{bootstrap_efron93,
  author = {Bradley Efron and Robert J. Tibshirani},
  publisher = {Chapman et Hall},
  title = {An {I}ntroduction to the {B}ootstrap},
  year = 1993
}
@inproceedings{aupetit2016design,
  title={A design study to identify inconsistencies in kinship information: The case of the 1000 Genomes project},
  author={ Micha{\"e}l Aupetit and Ehsan Ullah and Reda Rawi and Halima Bensmail},
  booktitle=PVIS,
  pages={254--258},
  year={2016},
  organization={IEEE}
}

@Manual{Rpackage_dbscan,
    title = {dbscan: Density Based Clustering of Applications with Noise (DBSCAN) and Related Algorithms},
    author = {Michael Hahsler and Matthew Piekenbrock},
    year = {2018},
    note = {R package version 1.1-3},
    url = {https://CRAN.R-project.org/package=dbscan},
  }

@Manual{Rpackage_subspace,
    title = {subspace: Interface to OpenSubspace},
    author = {Marwan Hassani and Matthias Hansen},
    year = {2015},
    note = {R package version 1.0.4},
    url = {https://CRAN.R-project.org/package=subspace},
  }
  
@article{Rpackage_RWeka,
    title = {Open-Source Machine Learning: R Meets Weka.},
    author = {K. Hornik and  C. Buchta and A. Zeileis},
    journal={Computational Statistics},
    volume={24},
    number={2},
    pages={225--232},
    year = {2009},
    url = {http://doi.org/10.1007/s00180-008-0119-7},
  }

@Manual{Rpackage_fpc,
    title = {fpc: Flexible Procedures for Clustering},
    author = {Christian Hennig},
    year = {2015},
    note = {R package version 2.1-10},
    url = {https://CRAN.R-project.org/package=fpc},
  }

  @Article{Rpackage_Rmixmod,
    title = {{Rmixmod}: The {R} Package of the Model-Based Unsupervised, Supervised, and Semi-Supervised Classification {Mixmod} Library},
    author = {R\'emi Lebret and Serge Iovleff and Florent Langrognet and Christophe Biernacki and Gilles Celeux and G\'erard Govaert},
    journal = {Journal of Statistical Software},
    year = {2015},
    volume = {67},
    number = {6},
    pages = {1--29},
    doi = {10.18637/jss.v067.i06},
    }
  
@ARTICLE{ProjPursuit_FriedmanTukey74, 
author={J. H. {Friedman} and J. W. {Tukey}}, 
journal=TOC, 
title={A Projection Pursuit Algorithm for Exploratory Data Analysis}, 
year={1974}, 
volume={C-23}, 
number={9}, 
pages={881-890}, 
doi={10.1109/T-C.1974.224051}, 
ISSN={0018-9340}, 
}



@ARTICLE{Irshad2015,
  title    = "Crowdsourcing image annotation for nucleus detection and
              segmentation in computational pathology: evaluating experts,
              automated methods, and the crowd",
  author   = "H. Irshad and L. Montaser-Kouhsari and G. Waltz and O. Bucur and J. A. Nowak and F. Dong and N. W. Knoblauch and A. H. Beck",
  journal  = "Pac Symp Biocomput",
  pages    = "294--305",
  year     =  2015,
  address  = "United States"
}

@ARTICLE{Dasgupta2010Pargnostics,
  author={Aritra Dasgupta and Robert Kosara},
  journal={IEEE Transactions on Visualization and Computer Graphics}, 
  title={Pargnostics: Screen-Space Metrics for Parallel Coordinates}, 
  year={2010},
  volume={16},
  number={6},
  pages={1017-1026},
  doi={10.1109/TVCG.2010.184}}

@inproceedings{Meyer2012TheFN,
  title={The four-level nested model revisited: blocks and guidelines},
  author={Miriah D. Meyer and Michael Sedlmair and Tamara Munzner},
  booktitle={Workshop on Beyond Time and Errors: Novel Evaluation Methods for Visualization},
  pages={},
  year={2012},
}

@ARTICLE{Munzner2009nestedModelEval,
  author={Tamara Munzner},
  journal={IEEE Transactions on Visualization and Computer Graphics}, 
  title={A Nested Model for Visualization Design and Validation}, 
  year={2009},
  volume={15},
  number={6},
  pages={921-928},
  doi={10.1109/TVCG.2009.111}}

@INPROCEEDINGS{Sim2003benchmarkStudy,
  author={S. E. Sim and S. Easterbrook and R. C. Holt},
  booktitle={25th International Conference on Software Engineering, 2003. Proceedings.}, 
  title={Using benchmarking to advance research: a challenge to software engineering}, 
  year={2003},
  volume={},
  number={},
  pages={74-83},
  doi={10.1109/ICSE.2003.1201189}}

@ARTICLE{Espadoto2021quantSurveyDR,
  author={Mateus Espadoto and Rafael M. Martins and Andreas Kerren and Nina S. T. Hirata and Alexandru C. Telea},
  journal={IEEE Transactions on Visualization and Computer Graphics}, 
  title={Toward a Quantitative Survey of Dimension Reduction Techniques}, 
  year={2021},
  volume={27},
  number={3},
  pages={2153-2173},
  doi={10.1109/TVCG.2019.2944182}}

@ARTICLE{Jeon2023CLAMS,
  author={Hyeon Jeon and Ghulam Jilani Quadri and Hyunwook Lee and Paul Rosen and Danielle Albers Szafir and Jinwook Seo},
  journal={IEEE Transactions on Visualization and Computer Graphics}, 
  title={CLAMS: A Cluster Ambiguity Measure for Estimating Perceptual Variability in Visual Clustering}, 
  year={2023},
  volume={},
  number={},
  pages={1-11},
  doi={10.1109/TVCG.2023.3327201}}


@ARTICLE{ZENODO_DATA,
  journal={Zenodo data repository}, 
  author={Mostafa M. Abbas and Micha{\"{e}}l Aupetit},
  title={Datasets and code for {ClustMe} and {ClustML} visual quality measures of grouping patterns in monochrome scatterplots}, 
  year={2023},
  url = {https://zenodo.org/records/10208143},
  doi={10.5281/zenodo.10208143}}

